Mapping the Multilingual Margins: Intersectional Biases of Sentiment Analysis Systems in English, Spanish, and Arabic

As natural language processing systems become more widespread, it is necessary to address fairness issues in their implementation and deployment to ensure that their negative impacts on society are understood and minimized. However, there is limited work that studies fairness using a multilingual and intersectional framework or on downstream tasks. In this paper, we introduce four multilingual Equity Evaluation Corpora, supplementary test sets designed to measure social biases, and a novel statistical framework for studying unisectional and intersectional social biases in natural language processing. We use these tools to measure gender, racial, ethnic, and intersectional social biases across five models trained on emotion regression tasks in English, Spanish, and Arabic. We find that many systems demonstrate statistically significant unisectional and intersectional social biases.

==> tables/Stats3.tex <==
\begin{table*}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{|ll|rrr|rrr|}
\hline
\multicolumn{2}{|c|}{}  & \multicolumn{3}{c|}{\textbf{Anger Coefficients}}  & \multicolumn{3}{c|}{\textbf{Fear Coefficients}} \\
  Language & Model & Race/Ethnicity & Gender & Intersection & Race/Ethnicity & Gender & Intersection \\ 
  \hline
   \textbf{English} & BERT+ & $0.008$ & $-0.021^{***}$ & $-0.028^{***}$ & $-0.023^{***}$ & $0.026^{***}$ & $-0.001$\\
   (Black-white) & mBERT & $0.014^{***}$ & $0.018^{***}$ & $-0.015^{***}$ & $-0.015^{***}$ & $0.037^{***}$ & $-0.017^{**}$\\
   &XLM-RoBERTa & $-0.001^{**}$ & $0.003^{***}$ & $-0.004^{***}$ & $-0.003^{***}$ & $0.003^{***}$ & $0.002$\\
   &SVM & $0.001$ & $0.002$ & $-0.001$  & $-0.001$ & $-0.0$ & $0.002$\\
   &fastText & $0.0$ & $-0.002$ & $-0.0$ & $-0.0$ & $0.001$ & $0.0$\\
   
   
   \textbf{English} & BERT+ & $0.005$ & $-0.014^{***}$ & $0.002$ & $0.01$ & $-0.02^{***}$ & $0.015^{*}$\\
   (Anglo-Latino)& mBERT & $0.014^{***}$ & $-0.014^{***}$ & $-0.005$ & $-0.034^{***}$ & $0.013^{***}$ & $0.007$\\
   &XLM-RoBERTa &  $-0.0$ & $0.002^{***}$ & $-0.002^{**}$  &  $0.0$ & $0.002^{**}$ & $0.0$\\
   &SVM & $-0.003$ & $0.001$ & $0.003$ & $-0.003$ & $0.003$ & $0.003$\\
   &fastText & $-0.0$ & $-0.001$ & $-0.0$ & $0.0$ & $0.001$ & $-0.0$ \\

    \textbf{Spanish} & BERT+ & $-0.011$ & $-0.006$ & $0.02^{*}$ & $-0.017^{*}$ & $-0.009$ & $0.042^{***}$\\
   & mBERT & $0.03^{***}$ & $-0.005^{*}$ & $0.006^{*}$ &  $0.026^{***}$ & $0.013^{***}$ & $-0.005^{*}$\\
   & XLM-RoBERTa & $0.003^{***}$ & $-0.002^{***}$ & $-0.002^{***}$ & $0.002^{***}$ & $-0.0$ & $-0.001^{**}$\\
   & SVM & $-0.004$ & $0.031^{***}$ & $0.004$ & $-0.002$ & $-0.006$ & $0.002$\\
   & fastText & $0.0$ & $0.053^{***}$ & $0.0$ & $-0.0$ & $-0.007$ & $0.0$\\

   \textbf{English} & BERT+ & $0.061^{***}$ & $-0.004$ & $-0.026^{***}$ & $0.037^{***}$ & $0.004$ & $-0.006$\\
   (Anglo-Arab)& mBERT & $-0.001$ & $-0.012^{***}$ & $0.022^{***}$  & $0.028^{***}$ & $0.029^{***}$ & $-0.041^{***}$\\
   & XLM-RoBERTa & $-0.002^{**}$ & $-0.003^{***}$ & $0.003^{***}$ & $-0.0$ & $-0.0$ & $0.001$\\
   & SVM & $0.001$ & $0.001$ & $-0.001$ & $0.002$ & $0.0$ & $-0.0$ \\
   & fastText & $-0.0$ & $-0.003$ & $-0.0$ & $-0.0$ & $0.0$ & $-0.0$\\
   
   
   \textbf{Arabic} & BERT+ & $-0.026^{***}$ & $-0.01^{**}$ & $0.007$ & $-0.016^{***}$ & $-0.004$ & $0.018^{***}$\\
   & mBERT & $0.004$ & $-0.008^{***}$ & $0.012^{***}$ & $0.002$ & $0.009^{***}$ & $-0.006^{*}$\\
   & XLM-RoBERTa & $-0.001^{*}$ & $-0.004^{***}$ & $0.001^{*}$ & $-0.002^{**}$ & $0.001$ & $0.0$ \\
   & SVM & $0.003$ & $-0.029^{***}$ & $0.01$  & $0.002$ & $-0.021^{***}$ & $0.008$\\
   & fastText & $-0.03^{***}$ & $-0.012^{**}$ & $0.019^{**}$  & $-0.018^{*}$ & $-0.031^{***}$ & $0.013$\\

   
   \hline
    \multicolumn{2}{|c|}{}  & \multicolumn{3}{c|}{\textbf{Joy Coefficients}}  & \multicolumn{3}{c|}{\textbf{Sadness Coefficients}} \\
  Language & Model & Race/Ethnicity & Gender & Intersection & Race/Ethnicity & Gender & Intersection \\ 

   \hline
   \textbf{English} & BERT+ & $-0.052^{***}$ & $-0.005$ & $0.028^{***}$ & $-0.017^{**}$ & $0.017^{**}$ & $0.007$ \\
   (Black-white)& mBERT & $0.003$ & $0.009^{*}$ & $0.002$ & $-0.025^{***}$ & $0.042^{***}$ & $-0.024^{***}$\\
   & XLM-RoBERTa & $-0.017^{***}$ & $0.002$ & $0.001$ & $-0.009^{***}$ & $0.002$ & $-0.001$ \\
   & SVM & $0.002$ & $0.0$ & $-0.001$ & $0.002$ & $0.002$ & $-0.002$ \\
   & fastText & $0.0$ & $0.001$ & $-0.0$ & $-0.0$ & $0.0$ & $-0.0$ \\
   
   \textbf{English} & BERT+ & $0.001$ & $-0.025^{***}$ & $0.016^{**}$ & $-0.005$ & $-0.013^{**}$ & $0.028^{***}$\\
   (Anglo-Latino)& mBERT & $0.005$ & $0.02^{***}$ & $0.017^{**}$  & $-0.006$ & $0.009^{*}$ & $0.011$\\
   & XLM-RoBERTa  & $0.002^{**}$ & $0.006^{***}$ & $0.0$  & $0.001$ & $-0.002^{**}$ & $0.001$\\
   & SVM & $-0.0$ & $-0.0$ & $0.0$  & $-0.002$ & $0.0$ & $0.002$\\
   & fastText & $-0.0$ & $0.001$ & $0.0$ & $0.0$ & $-0.0$ & $-0.0$\\
   
   \textbf{Spanish} & BERT+ & $0.012$ & $0.015^{*}$ & $-0.006$  & $0.004$ & $0.019^{**}$ & $0.004$\\
   & mBERT & $-0.021^{***}$ & $-0.008^{**}$ & $0.025^{***}$ & $0.016^{***}$ & $0.002$ & $-0.008$\\
   & XLM-RoBERTa & $-0.0$ & $0.002^{**}$ & $-0.001$  & $-0.0$ & $0.0$ & $-0.0$ \\
   & SVM & $0.002$ & $0.015^{***}$ & $-0.001$ & $-0.006$ & $0.006$ & $0.006$ \\
   & fastText & $-0.0$ & $-0.004$ & $-0.0$ & $0.0$ & $-0.002$ & $-0.0$ \\
    
    \textbf{English} & BERT+ & $0.047^{***}$ & $-0.004$ & $-0.019^{***}$ & $0.064^{***}$ & $-0.005$ & $-0.007$\\
   (Anglo-Arab)& mBERT & $-0.029^{***}$ & $0.023^{***}$ & $0.016^{**}$ & $0.0$ & $0.033^{***}$ & $-0.024^{**}$\\
   & XLM-RoBERTa & $-0.001$ & $0.001$ & $-0.0$ & $-0.001$ & $-0.002^{**}$ & $0.003^{***}$ \\
   & SVM & $0.0$ & $-0.002$ & $0.002$ & $0.004$ & $0.004$ & $-0.004$ \\
   & fastText & $-0.0$ & $0.001$ & $-0.0$ & $-0.0$ & $0.0$ & $-0.0$ \\

   \textbf{Arabic} & BERT+ & $-0.006$ & $0.016^{**}$ & $0.003$  & $0.034^{***}$ & $0.001$ & $-0.007$ \\
   & mBERT & $-0.001$ & $0.015^{***}$ & $0.002$  &  $0.027^{***}$ & $0.007^{*}$ & $-0.016^{***}$\\
   & XLM-RoBERTa & $-0.0$ & $-0.005^{**}$ & $0.005$  & $-0.0$ & $0.003^{*}$ & $-0.003$\\
   & SVM & $0.006$ & $-0.052^{***}$ & $0.023^{**}$ & $-0.002$ & $-0.031^{***}$ & $0.001$\\
   & fastText & $0.018^{**}$ & $-0.028^{***}$ & $0.018$ &  $-0.005$ & $-0.036^{***}$ & $0.031^{***}$ \\


   
   \hline
\end{tabular}}
\caption{Beta coefficients for EEC inference for all model, emotion, EEC combinations. Statistically significant results $(p \leq 0.01$) are marked with three asterisks ***, $(p \leq 0.05$) are marked with two asterisks **, $(p \leq 0.10$) are marked with one asterisk *}
\end{table*}


==> tables/anger.tex <==
\begin{table*}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{|c c c|c c c c|}
\hline
%\begin{table}[H]
%\centering
%\begin{tabular}{|c c|rrrrr|rrrrr|}
%  \hline
\multicolumn{3}{|c|}{}  & \multicolumn{4}{c|}{Beta Coefficient} \\
  Emotion & Language & Model & Baseline & Race & Gender & Intersection \\ 
  \hline
   Anger & English & BERT & $0.503^{***}$ & $0.008$ & $-0.021^{***}$ & $-0.028^{***}$\\
   && mBert & $0.426^{***}$ & $0.014^{***}$ & $0.018^{***}$ & $-0.015^{***}$\\
   && RoBERTa & $0.489^{***}$ & $-0.001^{**}$ & $0.003^{***}$ & $-0.004^{***}$\\
   && SVM & $0.513^{***}$ & $0.001$ & $0.002$ & $-0.001$\\
   && fastText & $0.498^{***}$ & $0.0$ & $-0.002$ & $-0.0$\\
   
   
   & English-Spanish & BERT & $0.435^{***}$ & $0.005$ & $-0.014^{***}$ & $0.002$\\
   && mBERT & $0.471^{***}$ & $0.014^{***}$ & $-0.014^{***}$ & $-0.005$\\
   && RoBERTa & $0.468^{***}$ & $-0.0$ & $0.002^{***}$ & $-0.002^{**}$\\
   && SVM & $0.514^{***}$ & $-0.003$ & $0.001$ & $0.003$\\
   && fastText & $0.534^{***}$ & $-0.0$ & $-0.001$ & $-0.0$\\
   
   & English-Arabic & BERT & $0.382^{***}$ & $0.061^{***}$ & $-0.004$ & $-0.026^{***}$ \\
   && mBERT & $0.45^{***}$ & $-0.001$ & $-0.012^{***}$ & $0.022^{***}$\\
   && RoBERTa &$0.475^{***}$ & $-0.002^{**}$ & $-0.003^{***}$ & $0.003^{***}$ \\
   && SVM &$0.514^{***}$ & $0.001$ & $0.001$ & $-0.001$ \\
   && fastText & $0.579^{***}$ & $-0.0$ & $-0.003$ & $-0.0$\\
   
   
   & Spanish & BERT & $0.453^{***}$ & $-0.011$ & $-0.006$ & $0.02^{*}$\\
   && mBERT & $0.426^{***}$ & $0.03^{***}$ & $-0.005^{*}$ & $0.006^{*}$\\
   && RoBERTa & $0.472^{***}$ & $0.003^{***}$ & $-0.002^{***}$ & $-0.002^{***}$\\
   && SVM &$0.494^{***}$ & $-0.004$ & $0.031^{***}$ & $0.004$ \\
   && fastText & $0.399^{***}$ & $0.0$ & $0.053^{***}$ & $0.0$\\
   
   & Arabic & BERT & $0.453^{***}$ & $-0.026^{***}$ & $-0.01^{**}$ & $0.007$\\
   && mBERT & $0.486^{***}$ & $0.004$ & $-0.008^{***}$ & $0.012^{***}$ \\
   && RoBERTa & $0.492^{***}$ & $-0.001^{*}$ & $-0.004^{***}$ & $0.001^{*}$\\
   && SVM & $0.497^{***}$ & $0.003$ & $-0.029^{***}$ & $0.01$\\
   && fastText &$0.418^{***}$ & $-0.03^{***}$ & $-0.012^{**}$ & $0.019^{**}$ \\

   
   \hline
   \hline
\end{tabular}}
\caption{Beta coefficients for Model EEC Predictions, with test statistics and corresponding p-values for the Angry emotion. Statistically significant results $(p \leq 0.01$) are marked with three asterisks ***, $(p \leq 0.05$) are marked with three asterisks **, $(p \leq 0.10$) are marked with three asterisks *}
\end{table*}


==> tables/baby_anger.tex <==
\begin{table*}[t]
\centering
\scalebox{0.6}{
\begin{tabular}{|c c|c c c c|}
\hline
%\begin{table}[H]
%\centering
%\begin{tabular}{|c|rrrrr|rrrrr|}
%  \hline
\multicolumn{2}{|c|}{}  & \multicolumn{4}{c|}{Beta Coefficient $b_i$} \\
  Language & Model & Intercept & Race/Ethnicity & Gender & Intersection \\ 
  \hline
   English & BERT & $0.503^{***}$ & $0.008$ & $-0.021^{***}$ & $-0.028^{***}$\\
   (Black-white) & mBert & $0.426^{***}$ & $0.014^{***}$ & $0.018^{***}$ & $-0.015^{***}$\\
   & RoBERTa & $0.489^{***}$ & $-0.001^{**}$ & $0.003^{***}$ & $-0.004^{***}$\\
   & SVM & $0.513^{***}$ & $0.001$ & $0.002$ & $-0.001$\\
   & fastText & $0.498^{***}$ & $0.0$ & $-0.002$ & $-0.0$\\
   
   English & BERT & $0.435^{***}$ & $0.005$ & $-0.014^{***}$ & $0.002$\\
   (Anglo-Latino) & mBERT & $0.471^{***}$ & $0.014^{***}$ & $-0.014^{***}$ & $-0.005$\\
   & RoBERTa & $0.468^{***}$ & $-0.0$ & $0.002^{***}$ & $-0.002^{**}$\\
   & SVM & $0.514^{***}$ & $-0.003$ & $0.001$ & $0.003$\\
   & fastText & $0.534^{***}$ & $-0.0$ & $-0.001$ & $-0.0$\\
  
    English & BERT & $0.382^{***}$ & $0.061^{***}$ & $-0.004$ & $-0.026^{***}$ \\
   (Anglo-Arab) & mBERT & $0.45^{***}$ & $-0.001$ & $-0.012^{***}$ & $0.022^{***}$\\
   & RoBERTa &$0.475^{***}$ & $-0.002^{**}$ & $-0.003^{***}$ & $0.003^{***}$ \\
   & SVM &$0.514^{***}$ & $0.001$ & $0.001$ & $-0.001$ \\
   & fastText & $0.579^{***}$ & $-0.0$ & $-0.003$ & $-0.0$\\
   
   
    Spanish & BERT & $0.453^{***}$ & $-0.011$ & $-0.006$ & $0.02^{*}$\\
   & mBERT & $0.426^{***}$ & $0.03^{***}$ & $-0.005^{*}$ & $0.006^{*}$\\
   & RoBERTa & $0.472^{***}$ & $0.003^{***}$ & $-0.002^{***}$ & $-0.002^{***}$\\
   & SVM &$0.494^{***}$ & $-0.004$ & $0.031^{***}$ & $0.004$ \\
   & fastText & $0.399^{***}$ & $0.0$ & $0.053^{***}$ & $0.0$\\
   
    Arabic & BERT & $0.453^{***}$ & $-0.026^{***}$ & $-0.01^{**}$ & $0.007$\\
   & mBERT & $0.486^{***}$ & $0.004$ & $-0.008^{***}$ & $0.012^{***}$ \\
   & RoBERTa & $0.492^{***}$ & $-0.001^{*}$ & $-0.004^{***}$ & $0.001^{*}$\\
   & SVM & $0.497^{***}$ & $0.003$ & $-0.029^{***}$ & $0.01$\\
   & fastText &$0.418^{***}$ & $-0.03^{***}$ & $-0.012^{**}$ & $0.019^{**}$ \\

   
   \hline
   \hline
\end{tabular}}
\caption{Beta coefficients for Model EEC Predictions, with test statistics and corresponding p-values for the Angry emotion. Statistically significant results $(p \leq 0.01$) are marked with three asterisks ***, $(p \leq 0.05$) are marked with three asterisks **, $(p \leq 0.10$) are marked with three asterisks *}
\end{table*}

==> tables/broken_results.tex <==
\begin{table}[t]
\centering
\scalebox{0.4}{
\begin{tabular}{|c c|c c c c|}
\hline
 & & \multicolumn{4}{c|}{\textbf{$\rho$ Test}}\\

  Language & Model & Anger & Fear & Joy & Sadness \\ 
  \hline
   \multirow{5}{*}{English} & BERT+ & 0.592&0.561&0.596&0.559\\ 
   & mBERT & 0.369&0.476&0.507&0.397\\
   & XLM-RoBERTa & 0.412&0.388&0.432&0.489\\ 
   & fastText & 0.535&0.467&0.495&0.452\\ 
   & SVM & 0.533&0.523&0.538&0.504\\ 
  \hline
\multirow{5}{*}{Spanish} & BERT+ &  0.391&0.460&0.555&0.459\\ 
   & mBERT & 0.279&0.192&0.510&0.367\\
   & XLM-RoBERTa &  0.136&0.358&0.329&0.145\\ 
   & fastText & 0.401&0.478&0.560&0.563\\ 
   & SVM & 0.398&0.638&0.551&0.598\\  
  \hline
  \multirow{5}{*}{Arabic} & BERT+ & 0.435&0.362&0.470&0.543 \\ 
   & mBERT & 0.223&0.111&0.296&0.384\\
   & XLM-RoBERTa &  0.211&0.254&0.212&0.139\\ 
   & fastText &  0.401&0.478&0.560&0.563\\ 
   & SVM &0.366&0.381&0.475&0.456 \\ 
\hline
\end{tabular}
}
\caption{Pearson Correlation Coefficent ($\rho$) on models trained on SemEval 2018 Task 1, Emotion Regression}
\label{tab:semresults}
\end{table}


% \begin{table}[t]
% % [!htbp]
% \centering
% \scalebox{0.7}{
% \begin{tabular}{|c c|c c c c|}
% \hline
% %\begin{table}[H]
% %\centering
% %\begin{tabular}{|c c|rrrrr|}
% %  \hline
% \multicolumn{2}{|c|}{}  & \multicolumn{4}{c|}{\textbf{$\rho$ Test}}\\
% %  Language & Model & Anger & Fear & Joy & Sadness & Valence & Anger & Fear & Joy & Sadness & Valence \\ 
% %  \hline
% %   English & BERT & 0.668 & 0.660 & 0.703& 0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
% %   & MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
% %   & XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
% %   & fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
% %   & SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\ 
% %  \hline
% %    Spanish & BERT &  0.521&0.628&0.689&0.607&0.665&0.391&0.460&0.555&0.459&0.564\\ 
% %   & MBERT & 0.309&0.346&0.538&0.470&0.457&0.279&0.192&0.510&0.367&0.380\\
% %   & XLM-RoBERTa &  0.212&0.421&0.335&0.228&0.521&0.136&0.358&0.329&0.145&0.484\\ 
% %   & fastText & 0.711&0.700&0.956&0.876&0.939&0.401&0.478&0.560&0.563&0.664 \\ 
% %   & SVM & 0.883&0.876&0.820&0.889&0.880&0.398&0.638&0.551&0.598&0.578\\  
% %  \hline
% %  Arabic & BERT & 0.550&0.498&0.559&0.661&0.684&0.435&0.362&0.470&0.543&0.642 \\ 
% %   & MBERT & 0.300&0.214&0.360&0.407&0.493&0.223&0.111&0.296&0.384&0.459\\
% %   & XLM-RoBERTa &  0.335&0.351&0.190&0.117&0.311&0.211&0.254&0.212&0.139&0.190\\ 
% %   & fastText &  0.711&0.700&0.956&0.876&0.939&0.401&0.478&0.560&0.563&0.664\\ 
% %   & SVM &0.846&0.900&0.946&0.883&0.918&0.366&0.381&0.475&0.456&0.583 \\ 
% %  \hline

%   Language & Model & Anger & Fear & Joy & Sadness \\ 
%   \hline
%   English & BERT+ & 0.592&0.561&0.596&0.559\\ 
%   & mBERT & 0.369&0.476&0.507&0.397\\
%   & XLM-RoBERTa & 0.412&0.388&0.432&0.489\\ 
%   & fastText & 0.535&0.467&0.495&0.452\\ 
%   & SVM & 0.533&0.523&0.538&0.504\\ 
%   \hline
%     Spanish & BERT+ &  0.391&0.460&0.555&0.459\\ 
%   & mBERT & 0.279&0.192&0.510&0.367\\
%   & XLM-RoBERTa &  0.136&0.358&0.329&0.145\\ 
%   & fastText & 0.401&0.478&0.560&0.563\\ 
%   & SVM & 0.398&0.638&0.551&0.598\\  
%   \hline
%   Arabic & BERT+ & 0.435&0.362&0.470&0.543 \\ 
%   & mBERT & 0.223&0.111&0.296&0.384\\
%   & XLM-RoBERTa &  0.211&0.254&0.212&0.139\\ 
%   & fastText &  0.401&0.478&0.560&0.563\\ 
%   & SVM &0.366&0.381&0.475&0.456 \\ 
% \hline
% \end{tabular}}
% \caption{Pearson Correlation Coefficent ($\rho$) on models trained on SemEval 2018 Task 1, Emotion Regression}
% \label{tab:semresults}
% \end{table}




==> tables/eec_templates.tex <==
% \setarab % choose the language specific conventions
% \vocalize % switch diacritics for short vowels on
%\transtrue % display the transliteration
% \arabtrue % print arabic text (on by default)
% \usepackage{utf8}
% \setcode{utf8}

\begin{table*}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{| l | l | l |}
\hline
Template & Example & EEC\\
\hline
% \bigstrut
1.[Person] feels [emotional state word].  & 
Adam feels angry.
& English (Black-white)
\\
\begin{tabular}[t]{@{}l@{}}2. The situation makes [person] feel\\ [emotional state word].\end{tabular} 
&
The situation makes Latoya feel excited.
& English (Black-white)
\\

3. I made [person] feel [emotional state word].
&
I made Jorge feel furious.
&
English (Latino-Anglo)
\\
4. [Person] made me feel [emotional state word].
&
Sarah made me feel depressed.
&
English (Latino-Anglo)
\\

\begin{tabular}[t]{@{}l@{}}5. [Person] found him/herself in a/an\\ [emotional situation word] situation. \end{tabular}
&
Ana se encontró en una situación maravillosa.
&
Spanish (Anglo-Latino)

\\
\begin{tabular}[t]{@{}l@{}}6. [Person] told us all about the recent\\ [emotional situation word] events.\end{tabular} 
&
Jacob nos contó todo sobre los recientes acontecimientos absurdos.
&
Spanish (Anglo-Latino)

\\
\begin{tabular}[t]{@{}l@{}}7. The conversation with [person] was\\ [emotional situation word] .\end{tabular}  
&
The conversation with Muhammad was hilarious.
&
English (Anglo-Arab)

\\
8. I saw [person] in the market.
&
I saw Betsy in the market.
&
English (Anglo-Arab)

\\
9. I talked to (person) yesterday.     
&

% \begin{arabtext}
% تحدثت مع جستين الأمس
% \end{arabtext}
% \setotherlanguage{arabic}
% \foreignlanguage{arabic}{
% \begin{otherlanguage}{arabic}
\< تحدثت مع جستين الأمس >
% تحدثت مع جستين الأمس
% }% \end{arabic}
% >
% \end{otherlanguage}
&
Arabic (Anglo-Arab)
\\


10. [Person] goes to the school in our neighborhood.
&
% \begin{arabtext}
% فاطمة تذهب إلى المدرسة في حينا 
% \end{arabtext}
\< فاطمة تذهب إلى المدرسة في حينا >
% \begin{otherlanguage}{arabic}
% فاطمة تذهب إلى المدرسة في حينا
% \end{otherlanguage}
% >
&
Arabic (Anglo-Arab)

\\
11. [Person] has two children.
&
my husband has two children.
&
English (all English EECs)
\\
\hline
\end{tabular}
}
\caption{Sentence templates used in the EECs}
\label{tab:eectemplates}
\end{table*}

==> tables/fear.tex <==
\begin{table*}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{|c c c|c c c c|}
\hline
%\begin{table}[H]
%\centering
%\begin{tabular}{|c c|rrrrr|rrrrr|}
%  \hline
\multicolumn{3}{|c|}{}  & \multicolumn{4}{c|}{Beta Coefficient} \\
  Emotion & Language & Model & Baseline & Race & Gender & Intersection \\ 
  \hline
   Fear & English & BERT &$0.516^{***}$ & $-0.023^{***}$ & $0.026^{***}$ & $-0.001$\\
   && mBert &$0.525^{***}$ & $-0.015^{***}$ & $0.037^{***}$ & $-0.017^{**}$\\
   && RoBERTa &$0.495^{***}$ & $-0.003^{***}$ & $0.003^{***}$ & $0.002$\\
   && SVM &$0.534^{***}$ & $-0.001$ & $-0.0$ & $0.002$\\
   && fastText &$0.545^{***}$ & $-0.0$ & $0.001$ & $0.0$\\
   
   & English-Spanish & BERT & $0.441^{***}$ & $0.01$ & $-0.02^{***}$ & $0.015^{*}$\\
   && mBERT & $0.524^{***}$ & $-0.034^{***}$ & $0.013^{***}$ & $0.007$\\
   && RoBERTa & $0.479^{***}$ & $0.0$ & $0.002^{**}$ & $0.0$\\
   && SVM & $0.533^{***}$ & $-0.003$ & $0.003$ & $0.003$\\
   && fastText & $0.612^{***}$ & $0.0$ & $0.001$ & $-0.0$ \\
   
   & English-Arabic & BERT & $0.46^{***}$ & $0.037^{***}$ & $0.004$ & $-0.006$\\
   && mBERT & $0.521^{***}$ & $0.028^{***}$ & $0.029^{***}$ & $-0.041^{***}$\\
   && RoBERTa & $0.475^{***}$ & $-0.0$ & $-0.0$ & $0.001$\\
   && SVM & $0.534^{***}$ & $0.002$ & $0.0$ & $-0.0$ \\
   && fastText & $0.621^{***}$ & $-0.0$ & $0.0$ & $-0.0$\\
   
   & Spanish & BERT & $0.524^{***}$ & $-0.017^{*}$ & $-0.009$ & $0.042^{***}$\\
   && mBERT & $0.495^{***}$ & $0.026^{***}$ & $0.013^{***}$ & $-0.005^{*}$\\
   && RoBERTa & $0.491^{***}$ & $0.002^{***}$ & $-0.0$ & $-0.001^{**}$\\
   && SVM & $0.488^{***}$ & $-0.002$ & $-0.006$ & $0.002$\\
   && fastText & $0.568^{***}$ & $-0.0$ & $-0.007$ & $0.0$\\
   
   & Arabic & BERT & $0.48^{***}$ & $-0.016^{***}$ & $-0.004$ & $0.018^{***}$\\
   && mBERT & $0.486^{***}$ & $0.002$ & $0.009^{***}$ & $-0.006^{*}$\\
   && RoBERTa &$0.504^{***}$ & $-0.002^{**}$ & $0.001$ & $0.0$ \\
   && SVM & $0.483^{***}$ & $0.002$ & $-0.021^{***}$ & $0.008$\\
   && fastText & $0.444^{***}$ & $-0.018^{*}$ & $-0.031^{***}$ & $0.013$\\

   \hline
\end{tabular}}
\caption{Beta coefficients for Model EEC Predictions, with test statistics and corresponding p-values for the Fear emotion. Statistically significant results $(p \leq 0.01$) are marked with three asterisks ***, $(p \leq 0.05$) are marked with three asterisks **, $(p \leq 0.10$) are marked with three asterisks *}
\end{table*}

==> tables/joy.tex <==
\begin{table*}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{|c c c|c c c c|}
\hline
%\begin{table}[H]
%\centering
%\begin{tabular}{|c c|rrrrr|rrrrr|}
%  \hline
\multicolumn{3}{|c|}{}  & \multicolumn{4}{c|}{Beta Coefficient} \\
  Emotion & Language & Model & Baseline & Race & Gender & Intersection \\ 
  \hline
   Joy & English & BERT &$0.463^{***}$ & $-0.052^{***}$ & $-0.005$ & $0.028^{***}$ \\
   && mBERT & $0.502^{***}$ & $0.003$ & $0.009^{*}$ & $0.002$\\
   && RoBERTa & $0.538^{***}$ & $-0.017^{***}$ & $0.002$ & $0.001$ \\
   && SVM & $0.556^{***}$ & $0.002$ & $0.0$ & $-0.001$\\
   && fastText & $0.53^{***}$ & $0.0$ & $0.001$ & $-0.0$ \\
   
   & English-Spanish & BERT & $0.45^{***}$ & $0.001$ & $-0.025^{***}$ & $0.016^{**}$\\
   && mBERT & $0.45^{***}$ & $0.005$ & $0.02^{***}$ & $0.017^{**}$\\
   && RoBERTa & $0.464^{***}$ & $0.002^{**}$ & $0.006^{***}$ & $0.0$\\
   && SVM & $0.558^{***}$ & $-0.0$ & $-0.0$ & $0.0$ \\
   && fastText & $0.589^{***}$ & $-0.0$ & $0.001$ & $0.0$\\
   
   & English-Arabic & BERT & $0.426^{***}$ & $0.047^{***}$ & $-0.004$ & $-0.019^{***}$\\
   && mBERT & $0.475^{***}$ & $-0.029^{***}$ & $0.023^{***}$ & $0.016^{**}$\\
   && RoBERTa & $0.443^{***}$ & $-0.001$ & $0.001$ & $-0.0$\\
   && SVM & $0.558^{***}$ & $0.0$ & $-0.002$ & $0.002$\\
   && fastText & $0.628^{***}$ & $-0.0$ & $0.001$ & $-0.0$\\
   
   & Spanish & BERT & $0.548^{***}$ & $0.012$ & $0.015^{*}$ & $-0.006$\\
   && mBERT & $0.475^{***}$ & $-0.021^{***}$ & $-0.008^{**}$ & $0.025^{***}$\\
   && RoBERTa &$0.453^{***}$ & $-0.0$ & $0.002^{**}$ & $-0.001$ \\
   && SVM & $0.486^{***}$ & $0.002$ & $0.015^{***}$ & $-0.001$\\
   && fastText & $0.54^{***}$ & $-0.0$ & $-0.004$ & $-0.0$\\
   
   & Arabic & BERT & $0.458^{***}$ & $-0.006$ & $0.016^{**}$ & $0.003$\\
   && mBERT & $0.441^{***}$ & $-0.001$ & $0.015^{***}$ & $0.002$\\
   && RoBERTa & $0.473^{***}$ & $-0.0$ & $-0.005^{**}$ & $0.005$\\
   && SVM & $0.453^{***}$ & $0.006$ & $-0.052^{***}$ & $0.023^{**}$\\
   && fastText &$0.415^{***}$ & $0.018^{**}$ & $-0.028^{***}$ & $0.018$ \\
   \hline
\end{tabular}}
\caption{Beta coefficients for Model EEC Predictions, with test statistics and corresponding p-values for the Joy emotion. Statistically significant results $(p \leq 0.01$) are marked with three asterisks ***, $(p \leq 0.05$) are marked with three asterisks **, $(p \leq 0.10$) are marked with three asterisks *}
\end{table*}

==> tables/name.tex <==



==> tables/results_withtrain.tex <==

\begin{table*}[t]
%[!htbp]
\centering
\scalebox{0.7}{
\begin{tabular}{|c c|c c c c| c c c c |}
\hline
%\begin{table}[H]
%\centering
%\begin{tabular}{|c c|rrrrr|rrrrr|}
%  \hline
\multicolumn{2}{|c|}{}  & \multicolumn{4}{c|}{\textbf{$\rho$ Train}}  & \multicolumn{4}{c|}{\textbf{$\rho$ Test}}\\
%  Language & Model & Anger & Fear & Joy & Sadness & Valence & Anger & Fear & Joy & Sadness & Valence \\ 
%  \hline
%   English & BERT & 0.668 & 0.660 & 0.703& 0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
%   & MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
%   & XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
%   & fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
%   & SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\ 
%  \hline
%    Spanish & BERT &  0.521&0.628&0.689&0.607&0.665&0.391&0.460&0.555&0.459&0.564\\ 
%   & MBERT & 0.309&0.346&0.538&0.470&0.457&0.279&0.192&0.510&0.367&0.380\\
%   & XLM-RoBERTa &  0.212&0.421&0.335&0.228&0.521&0.136&0.358&0.329&0.145&0.484\\ 
%   & fastText & 0.711&0.700&0.956&0.876&0.939&0.401&0.478&0.560&0.563&0.664 \\ 
%   & SVM & 0.883&0.876&0.820&0.889&0.880&0.398&0.638&0.551&0.598&0.578\\  
%  \hline
%  Arabic & BERT & 0.550&0.498&0.559&0.661&0.684&0.435&0.362&0.470&0.543&0.642 \\ 
%   & MBERT & 0.300&0.214&0.360&0.407&0.493&0.223&0.111&0.296&0.384&0.459\\
%   & XLM-RoBERTa &  0.335&0.351&0.190&0.117&0.311&0.211&0.254&0.212&0.139&0.190\\ 
%   & fastText &  0.711&0.700&0.956&0.876&0.939&0.401&0.478&0.560&0.563&0.664\\ 
%   & SVM &0.846&0.900&0.946&0.883&0.918&0.366&0.381&0.475&0.456&0.583 \\ 
%  \hline

  Language & Model & Anger & Fear & Joy & Sadness & Anger & Fear & Joy & Sadness  \\ 
  \hline
   English & BERT & 0.668 & 0.660 & 0.703& 0.668&0.592&0.561&0.596&0.559\\ 
   & mBERT & 0.518&0.589&0.624&0.581&0.369&0.476&0.507&0.397\\
   & XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.412&0.388&0.432&0.489\\ 
   & fastText & 0.960&0.667&0.665&0.691&0.535&0.467&0.495&0.452\\ 
   & SVM & 0.880&0.939&0.949&0.817&0.533&0.523&0.538&0.504\\ 
  \hline
    Spanish & BERT &  0.521&0.628&0.689&0.607&0.391&0.460&0.555&0.459\\ 
   & mBERT & 0.309&0.346&0.538&0.470&0.279&0.192&0.510&0.367\\
   & XLM-RoBERTa &  0.212&0.421&0.335&0.228&0.136&0.358&0.329&0.145\\ 
   & fastText & 0.711&0.700&0.956&0.876&0.401&0.478&0.560&0.563\\ 
   & SVM & 0.883&0.876&0.820&0.889&0.398&0.638&0.551&0.598\\  
  \hline
  Arabic & BERT & 0.550&0.498&0.559&0.661&0.435&0.362&0.470&0.543 \\ 
   & mBERT & 0.300&0.214&0.360&0.407&0.223&0.111&0.296&0.384\\
   & XLM-RoBERTa &  0.335&0.351&0.190&0.117&0.211&0.254&0.212&0.139\\ 
   & fastText &  0.711&0.700&0.956&0.876&0.401&0.478&0.560&0.563\\ 
   & SVM &0.846&0.900&0.946&0.883&0.366&0.381&0.475&0.456 \\ 
\hline
\end{tabular}}
\caption{Pearson Correlation Coefficent ($\rho$) on models trained on SemEval 2018 Task 1, Emotion Regression}
\label{tab:semresults}
\end{table*}



==> tables/sadness.tex <==
\begin{table*}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{|c c c|c c c c|}
\hline
%\begin{table}[H]
%\centering
%\begin{tabular}{|c c|rrrrr|rrrrr|}
%  \hline
\multicolumn{3}{|c|}{}  & \multicolumn{4}{c|}{Beta Coefficient} \\
  Emotion & Language & Model & Baseline & Race & Gender & Intersection \\ 
  \hline
Sadness & English & BERT &$0.509^{***}$ & $-0.017^{**}$ & $0.017^{**}$ & $0.007$ \\
   && mBERT & $0.522^{***}$ & $-0.025^{***}$ & $0.042^{***}$ & $-0.024^{***}$\\
   && RoBERTa &$0.516^{***}$ & $-0.009^{***}$ & $0.002$ & $-0.001$ \\
   && SVM &$0.557^{***}$ & $0.002$ & $0.002$ & $-0.002$ \\
   && fastText &$0.505^{***}$ & $-0.0$ & $0.0$ & $-0.0$ \\
   
   & English-Spanish & BERT & $0.478^{***}$ & $-0.005$ & $-0.013^{**}$ & $0.028^{***}$\\
   && mBERT & $0.55^{***}$ & $-0.006$ & $0.009^{*}$ & $0.011$\\
   && RoBERTa & $0.472^{***}$ & $0.001$ & $-0.002^{**}$ & $0.001$\\
   && SVM & $0.559^{***}$ & $-0.002$ & $0.0$ & $0.002$\\
   && fastText & $0.605^{***}$ & $0.0$ & $-0.0$ & $-0.0$\\
   
   & English-Arabic & BERT & $0.422^{***}$ & $0.064^{***}$ & $-0.005$ & $-0.007$\\
   && mBERT & $0.559^{***}$ & $0.0$ & $0.033^{***}$ & $-0.024^{**}$\\
   && RoBERTa &$0.496^{***}$ & $-0.001$ & $-0.002^{**}$ & $0.003^{***}$ \\
   && SVM &$0.555^{***}$ & $0.004$ & $0.004$ & $-0.004$ \\
   && fastText &$0.6^{***}$ & $-0.0$ & $0.0$ & $-0.0$ \\
   
   & Spanish & BERT & $0.53^{***}$ & $0.004$ & $0.019^{**}$ & $0.004$\\
   && mBERT & $0.479^{***}$ & $0.016^{***}$ & $0.002$ & $-0.008$\\
   && RoBERTa & $0.462^{***}$ & $-0.0$ & $0.0$ & $-0.0$ \\
   && SVM & $0.552^{***}$ & $-0.006$ & $0.006$ & $0.006$ \\
   && fastText & $0.588^{***}$ & $0.0$ & $-0.002$ & $-0.0$ \\
   
   & Arabic & BERT &$0.467^{***}$ & $0.034^{***}$ & $0.001$ & $-0.007$ \\
   && mBERT & $0.469^{***}$ & $0.027^{***}$ & $0.007^{*}$ & $-0.016^{***}$\\
   && RoBERTa & $0.479^{***}$ & $-0.0$ & $0.003^{*}$ & $-0.003$\\
   && SVM & $0.533^{***}$ & $-0.002$ & $-0.031^{***}$ & $0.001$\\
   && fastText & $0.476^{***}$ & $-0.005$ & $-0.036^{***}$ & $0.031^{***}$ \\
   \hline
\end{tabular}}
\caption{Beta coefficients for Model EEC Predictions, with test statistics and corresponding p-values for the Sadness emotion. Statistically significant results $(p \leq 0.01$) are marked with three asterisks ***, $(p \leq 0.05$) are marked with three asterisks **, $(p \leq 0.10$) are marked with three asterisks *}
\end{table*}


==> tables/stats.tex <==
\begin{table*}[t]
\centering
\scalebox{0.5}{
\begin{tabular}{|c c c |rrrr|rrrr|rrrr|}
\hline
%\begin{table}[H]
%\centering
%\begin{tabular}{|c c|rrrrr|rrrrr|}
%  \hline
& \multicolumn{9}{c}{Beta Coefficient} & \multicolumn{2}{c}{Test Statistic} & \multicolumn{2}{c}{p-value} \\
  Emotion & Language & Model & Baseline & Race & Gender & Intersectionality & Baseline & Race & Gender & Intersectionality & Baseline & Race & Gender & Intersectionality \\ 
  \hline
   Anger & English & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\ 
   & Spanish & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\ 
   & Arabic & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   & Spanish & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\ 
   & Arabic & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\
   
  \hline
  Fear & English & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\ 
   & Spanish & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\ 
   & Arabic & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\
  \hline
  Joy & English & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\ 
   & Spanish & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\ 
   & Arabic & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\
  \hline
  Sadness & English & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\ 
   & Spanish & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\ 
   & Arabic & BERT & 0.668 & 0.660 & 0.703& &&0.668&0.674&0.592&0.561&0.596&0.559	&0.614\\ 
   && MBERT & 0.518&0.589&0.624&0.581&0.549&0.369&0.476&0.507&0.397&0.507 \\
   && XLM-RoBERTa & 0.506&0.532&0.504&0.564&0.296&0.412&0.388&0.432&0.489&0.314 \\ 
   && fastText & 0.960&0.667&0.665&0.691&0.912&0.535&0.467&0.495&0.452&0.573 \\ 
   && SVM & 0.880&0.939&0.949&0.817&0.936&0.533&0.523&0.538&0.504&0.595\\
  \hline
\end{tabular}}
\caption{Beta coefficients for Model EEC Predictions, with test statistics and corresponding p-values. Statistically significant results $(p \leq 0.05$) are marked with an asterisk *}
\end{table*}


==> tables/stats_2.tex <==
\begin{table*}[t]
\centering
\scalebox{0.6}{
\begin{tabular}{|c c c|c c c c|}
\hline
%\begin{table}[H]
%\centering
%\begin{tabular}{|c c|rrrrr|rrrrr|}
%  \hline
\multicolumn{3}{|c|}{}  & \multicolumn{4}{c|}{Beta Coefficient} \\
  Emotion & Language & Model & Intercept & Race & Gender & Intersection \\ 
  \hline
   Anger & English & BERT & $0.503^{***}$ & $0.008$ & $-0.021^{***}$ & $-0.028^{***}$\\
   & (Black-white) & mBert & $0.426^{***}$ & $0.014^{***}$ & $0.018^{***}$ & $-0.015^{***}$\\
   && RoBERTa & $0.489^{***}$ & $-0.001^{**}$ & $0.003^{***}$ & $-0.004^{***}$\\
   && SVM & $0.513^{***}$ & $0.001$ & $0.002$ & $-0.001$\\
   && fastText & $0.498^{***}$ & $0.0$ & $-0.002$ & $-0.0$\\
   
   
   & English & BERT & $0.435^{***}$ & $0.005$ & $-0.014^{***}$ & $0.002$\\
   &(Anglo-Latino)& mBERT & $0.471^{***}$ & $0.014^{***}$ & $-0.014^{***}$ & $-0.005$\\
   && RoBERTa & $0.468^{***}$ & $-0.0$ & $0.002^{***}$ & $-0.002^{**}$\\
   && SVM & $0.514^{***}$ & $-0.003$ & $0.001$ & $0.003$\\
   && fastText & $0.534^{***}$ & $-0.0$ & $-0.001$ & $-0.0$\\
   
   & English-Arabic & BERT & $0.382^{***}$ & $0.061^{***}$ & $-0.004$ & $-0.026^{***}$ \\
   &(Anglo-Arab)& mBERT & $0.45^{***}$ & $-0.001$ & $-0.012^{***}$ & $0.022^{***}$\\
   && RoBERTa &$0.475^{***}$ & $-0.002^{**}$ & $-0.003^{***}$ & $0.003^{***}$ \\
   && SVM &$0.514^{***}$ & $0.001$ & $0.001$ & $-0.001$ \\
   && fastText & $0.579^{***}$ & $-0.0$ & $-0.003$ & $-0.0$\\
   
   
   & Spanish & BERT & $0.453^{***}$ & $-0.011$ & $-0.006$ & $0.02^{*}$\\
   && mBERT & $0.426^{***}$ & $0.03^{***}$ & $-0.005^{*}$ & $0.006^{*}$\\
   && RoBERTa & $0.472^{***}$ & $0.003^{***}$ & $-0.002^{***}$ & $-0.002^{***}$\\
   && SVM &$0.494^{***}$ & $-0.004$ & $0.031^{***}$ & $0.004$ \\
   && fastText & $0.399^{***}$ & $0.0$ & $0.053^{***}$ & $0.0$\\
   
   & Arabic & BERT & $0.453^{***}$ & $-0.026^{***}$ & $-0.01^{**}$ & $0.007$\\
   && mBERT & $0.486^{***}$ & $0.004$ & $-0.008^{***}$ & $0.012^{***}$ \\
   && RoBERTa & $0.492^{***}$ & $-0.001^{*}$ & $-0.004^{***}$ & $0.001^{*}$\\
   && SVM & $0.497^{***}$ & $0.003$ & $-0.029^{***}$ & $0.01$\\
   && fastText &$0.418^{***}$ & $-0.03^{***}$ & $-0.012^{**}$ & $0.019^{**}$ \\

   
   \hline
   Fear & English & BERT &$0.516^{***}$ & $-0.023^{***}$ & $0.026^{***}$ & $-0.001$\\
   &(Black-white)& mBert &$0.525^{***}$ & $-0.015^{***}$ & $0.037^{***}$ & $-0.017^{**}$\\
   && RoBERTa &$0.495^{***}$ & $-0.003^{***}$ & $0.003^{***}$ & $0.002$\\
   && SVM &$0.534^{***}$ & $-0.001$ & $-0.0$ & $0.002$\\
   && fastText &$0.545^{***}$ & $-0.0$ & $0.001$ & $0.0$\\
   
   & English-Spanish & BERT & $0.441^{***}$ & $0.01$ & $-0.02^{***}$ & $0.015^{*}$\\
   &(Anglo-Latino)& mBERT & $0.524^{***}$ & $-0.034^{***}$ & $0.013^{***}$ & $0.007$\\
   && RoBERTa & $0.479^{***}$ & $0.0$ & $0.002^{**}$ & $0.0$\\
   && SVM & $0.533^{***}$ & $-0.003$ & $0.003$ & $0.003$\\
   && fastText & $0.612^{***}$ & $0.0$ & $0.001$ & $-0.0$ \\
   
   & English-Arabic & BERT & $0.46^{***}$ & $0.037^{***}$ & $0.004$ & $-0.006$\\
   &(Anglo-Arab)& mBERT & $0.521^{***}$ & $0.028^{***}$ & $0.029^{***}$ & $-0.041^{***}$\\
   && RoBERTa & $0.475^{***}$ & $-0.0$ & $-0.0$ & $0.001$\\
   && SVM & $0.534^{***}$ & $0.002$ & $0.0$ & $-0.0$ \\
   && fastText & $0.621^{***}$ & $-0.0$ & $0.0$ & $-0.0$\\
   
   & Spanish & BERT & $0.524^{***}$ & $-0.017^{*}$ & $-0.009$ & $0.042^{***}$\\
   && mBERT & $0.495^{***}$ & $0.026^{***}$ & $0.013^{***}$ & $-0.005^{*}$\\
   && RoBERTa & $0.491^{***}$ & $0.002^{***}$ & $-0.0$ & $-0.001^{**}$\\
   && SVM & $0.488^{***}$ & $-0.002$ & $-0.006$ & $0.002$\\
   && fastText & $0.568^{***}$ & $-0.0$ & $-0.007$ & $0.0$\\
   
   & Arabic & BERT & $0.48^{***}$ & $-0.016^{***}$ & $-0.004$ & $0.018^{***}$\\
   && mBERT & $0.486^{***}$ & $0.002$ & $0.009^{***}$ & $-0.006^{*}$\\
   && RoBERTa &$0.504^{***}$ & $-0.002^{**}$ & $0.001$ & $0.0$ \\
   && SVM & $0.483^{***}$ & $0.002$ & $-0.021^{***}$ & $0.008$\\
   && fastText & $0.444^{***}$ & $-0.018^{*}$ & $-0.031^{***}$ & $0.013$\\

   \hline
   Joy & English & BERT &$0.463^{***}$ & $-0.052^{***}$ & $-0.005$ & $0.028^{***}$ \\
   &(Black-white)& mBERT & $0.502^{***}$ & $0.003$ & $0.009^{*}$ & $0.002$\\
   && RoBERTa & $0.538^{***}$ & $-0.017^{***}$ & $0.002$ & $0.001$ \\
   && SVM & $0.556^{***}$ & $0.002$ & $0.0$ & $-0.001$\\
   && fastText & $0.53^{***}$ & $0.0$ & $0.001$ & $-0.0$ \\
   
   & English & BERT & $0.45^{***}$ & $0.001$ & $-0.025^{***}$ & $0.016^{**}$\\
   &(Anglo-Latino)& mBERT & $0.45^{***}$ & $0.005$ & $0.02^{***}$ & $0.017^{**}$\\
   && RoBERTa & $0.464^{***}$ & $0.002^{**}$ & $0.006^{***}$ & $0.0$\\
   && SVM & $0.558^{***}$ & $-0.0$ & $-0.0$ & $0.0$ \\
   && fastText & $0.589^{***}$ & $-0.0$ & $0.001$ & $0.0$\\
   
   & English & BERT & $0.426^{***}$ & $0.047^{***}$ & $-0.004$ & $-0.019^{***}$\\
   &(Anglo-Arab)& mBERT & $0.475^{***}$ & $-0.029^{***}$ & $0.023^{***}$ & $0.016^{**}$\\
   && RoBERTa & $0.443^{***}$ & $-0.001$ & $0.001$ & $-0.0$\\
   && SVM & $0.558^{***}$ & $0.0$ & $-0.002$ & $0.002$\\
   && fastText & $0.628^{***}$ & $-0.0$ & $0.001$ & $-0.0$\\
   
   & Spanish & BERT & $0.548^{***}$ & $0.012$ & $0.015^{*}$ & $-0.006$\\
   && mBERT & $0.475^{***}$ & $-0.021^{***}$ & $-0.008^{**}$ & $0.025^{***}$\\
   && RoBERTa &$0.453^{***}$ & $-0.0$ & $0.002^{**}$ & $-0.001$ \\
   && SVM & $0.486^{***}$ & $0.002$ & $0.015^{***}$ & $-0.001$\\
   && fastText & $0.54^{***}$ & $-0.0$ & $-0.004$ & $-0.0$\\
   
   & Arabic & BERT & $0.458^{***}$ & $-0.006$ & $0.016^{**}$ & $0.003$\\
   && mBERT & $0.441^{***}$ & $-0.001$ & $0.015^{***}$ & $0.002$\\
   && RoBERTa & $0.473^{***}$ & $-0.0$ & $-0.005^{**}$ & $0.005$\\
   && SVM & $0.453^{***}$ & $0.006$ & $-0.052^{***}$ & $0.023^{**}$\\
   && fastText &$0.415^{***}$ & $0.018^{**}$ & $-0.028^{***}$ & $0.018$ \\

   
  \hline
Sadness & English & BERT &$0.509^{***}$ & $-0.017^{**}$ & $0.017^{**}$ & $0.007$ \\
   &(Black-white)& mBERT & $0.522^{***}$ & $-0.025^{***}$ & $0.042^{***}$ & $-0.024^{***}$\\
   && RoBERTa &$0.516^{***}$ & $-0.009^{***}$ & $0.002$ & $-0.001$ \\
   && SVM &$0.557^{***}$ & $0.002$ & $0.002$ & $-0.002$ \\
   && fastText &$0.505^{***}$ & $-0.0$ & $0.0$ & $-0.0$ \\
   
   & English & BERT & $0.478^{***}$ & $-0.005$ & $-0.013^{**}$ & $0.028^{***}$\\
   &(Anglo-Latino)& mBERT & $0.55^{***}$ & $-0.006$ & $0.009^{*}$ & $0.011$\\
   && RoBERTa & $0.472^{***}$ & $0.001$ & $-0.002^{**}$ & $0.001$\\
   && SVM & $0.559^{***}$ & $-0.002$ & $0.0$ & $0.002$\\
   && fastText & $0.605^{***}$ & $0.0$ & $-0.0$ & $-0.0$\\
   
   & English & BERT & $0.422^{***}$ & $0.064^{***}$ & $-0.005$ & $-0.007$\\
   &(Anglo-Arab)& mBERT & $0.559^{***}$ & $0.0$ & $0.033^{***}$ & $-0.024^{**}$\\
   && RoBERTa &$0.496^{***}$ & $-0.001$ & $-0.002^{**}$ & $0.003^{***}$ \\
   && SVM &$0.555^{***}$ & $0.004$ & $0.004$ & $-0.004$ \\
   && fastText &$0.6^{***}$ & $-0.0$ & $0.0$ & $-0.0$ \\
   
   & Spanish & BERT & $0.53^{***}$ & $0.004$ & $0.019^{**}$ & $0.004$\\
   && mBERT & $0.479^{***}$ & $0.016^{***}$ & $0.002$ & $-0.008$\\
   && RoBERTa & $0.462^{***}$ & $-0.0$ & $0.0$ & $-0.0$ \\
   && SVM & $0.552^{***}$ & $-0.006$ & $0.006$ & $0.006$ \\
   && fastText & $0.588^{***}$ & $0.0$ & $-0.002$ & $-0.0$ \\
   
   & Arabic & BERT &$0.467^{***}$ & $0.034^{***}$ & $0.001$ & $-0.007$ \\
   && mBERT & $0.469^{***}$ & $0.027^{***}$ & $0.007^{*}$ & $-0.016^{***}$\\
   && RoBERTa & $0.479^{***}$ & $-0.0$ & $0.003^{*}$ & $-0.003$\\
   && SVM & $0.533^{***}$ & $-0.002$ & $-0.031^{***}$ & $0.001$\\
   && fastText & $0.476^{***}$ & $-0.005$ & $-0.036^{***}$ & $0.031^{***}$ \\

 \hline
    Valence & English & BERT & $0.458^{***}$ & $-0.039$ & $-0.005$ & $0.048$
\\
       && mBERT & $0.495^{***}$ & $-0.004$ & $0.013$ & $0.01$\\
       && RoBERTa & $0.563^{***}$ & $-0.019^{**}$ & $-0.012$ & $-0.001$\\
       && SVM & $0.485^{***}$ & $0.007$ & $0.007$ & $-0.007$\\
       && fastText & $0.441^{***}$ & $-0.0$ & $0.0$ & $-0.0$\\
       
   & English & BERT & $0.445^{***}$ & $-0.005$ & $-0.005$ & $0.002$\\
   &Anglo-Latino& mBERT & $0.507^{***}$ & $-0.001$ & $0.006$ & $0.011$\\
   && RoBERTa & $0.48^{***}$ & $-0.002$ & $-0.003$ & $-0.002$\\
   && SVM &$0.489^{***}$ & $0.001$ & $0.003$ & $-0.001$ \\
   && fastText & $0.541^{***}$ & $-0.0$ & $0.0$ & $-0.0$\\
   
   & English-Arabic & BERT & $0.378^{***}$ & $0.027^{**}$ & $-0.059^{***}$ & $0.029$\\
   &Anglo-Arab& mBERT & $0.503^{***}$ & $-0.012$ & $-0.008$ & $0.016$\\
   && RoBERTa & $0.468^{***}$ & $-0.001$ & $-0.002$ & $-0.002$ \\
   && SVM & $0.492^{***}$ & $0.0$ & $-0.0$ & $-0.0$\\
   && fastText & $0.528^{***}$ & $-0.0$ & $0.0$ & $0.0$\\
   
   
   & Spanish & BERT & $0.427^{***}$ & $-0.033^{*}$ & $0.012$ & $-0.023$\\
   && mBERT & $0.523^{***}$ & $0.028^{**}$ & $0.01$ & $-0.011$\\
   && RoBERTa &$0.493^{***}$ & $-0.002$ & $0.001$ & $0.001$ \\
   && SVM &$0.507^{***}$ & $0.0$ & $-0.0$ & $0.0$ \\
   && fastText & $0.564^{***}$ & $0.0$ & $-0.0$ & $-0.0$\\
   
   & Arabic & BERT & $0.532^{***}$ & $0.021^{*}$ & $0.06^{***}$ & $-0.052^{***}$\\
   && mBERT & $0.423^{***}$ & $0.015$ & $0.005$ & $-0.002$\\
   && RoBERTa & $0.414^{***}$ & $-0.002$ & $-0.008$ & $0.003$\\
   && SVM & $0.472^{***}$ & $0.002$ & $0.003$ & $0.03^{*}$\\
   && fastText & $0.414^{***}$ & $0.07^{***}$ & $0.033^{**}$ & $-0.034$\\

   
   \hline
\end{tabular}}
\caption{Beta coefficients for Model EEC Predictions, with test statistics and corresponding p-values. Statistically significant results $(p \leq 0.05$) are marked with an asterisk *}
\end{table*}


==> tables/valence.tex <==
\begin{table*}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{|c c c|c c c c|}
\hline
%\begin{table}[H]
%\centering
%\begin{tabular}{|c c|rrrrr|rrrrr|}
%  \hline
\multicolumn{3}{|c|}{}  & \multicolumn{4}{c|}{Beta Coefficient} \\
  Emotion & Language & Model & Baseline & Race & Gender & Intersection \\ 
 \hline
    Valence & English & BERT & $0.458^{***}$ & $-0.039$ & $-0.005$ & $0.048$
\\
       && mBERT & $0.495^{***}$ & $-0.004$ & $0.013$ & $0.01$\\
       && RoBERTa & $0.563^{***}$ & $-0.019^{**}$ & $-0.012$ & $-0.001$\\
       && SVM & $0.485^{***}$ & $0.007$ & $0.007$ & $-0.007$\\
       && fastText & $0.441^{***}$ & $-0.0$ & $0.0$ & $-0.0$\\
       
   & English-Spanish & BERT & $0.445^{***}$ & $-0.005$ & $-0.005$ & $0.002$\\
   && mBERT & $0.507^{***}$ & $-0.001$ & $0.006$ & $0.011$\\
   && RoBERTa & $0.48^{***}$ & $-0.002$ & $-0.003$ & $-0.002$\\
   && SVM &$0.489^{***}$ & $0.001$ & $0.003$ & $-0.001$ \\
   && fastText & $0.541^{***}$ & $-0.0$ & $0.0$ & $-0.0$\\
   
   & English-Arabic & BERT & $0.378^{***}$ & $0.027^{**}$ & $-0.059^{***}$ & $0.029$\\
   && mBERT & $0.503^{***}$ & $-0.012$ & $-0.008$ & $0.016$\\
   && RoBERTa & $0.468^{***}$ & $-0.001$ & $-0.002$ & $-0.002$ \\
   && SVM & $0.492^{***}$ & $0.0$ & $-0.0$ & $-0.0$\\
   && fastText & $0.528^{***}$ & $-0.0$ & $0.0$ & $0.0$\\
   
   
   & Spanish & BERT & $0.427^{***}$ & $-0.033^{*}$ & $0.012$ & $-0.023$\\
   && mBERT & $0.523^{***}$ & $0.028^{**}$ & $0.01$ & $-0.011$\\
   && RoBERTa &$0.493^{***}$ & $-0.002$ & $0.001$ & $0.001$ \\
   && SVM &$0.507^{***}$ & $0.0$ & $-0.0$ & $0.0$ \\
   && fastText & $0.564^{***}$ & $0.0$ & $-0.0$ & $-0.0$\\
   
   & Arabic & BERT & $0.532^{***}$ & $0.021^{*}$ & $0.06^{***}$ & $-0.052^{***}$\\
   && mBERT & $0.423^{***}$ & $0.015$ & $0.005$ & $-0.002$\\
   && RoBERTa & $0.414^{***}$ & $-0.002$ & $-0.008$ & $0.003$\\
   && SVM & $0.472^{***}$ & $0.002$ & $0.003$ & $0.03^{*}$\\
   && fastText & $0.414^{***}$ & $0.07^{***}$ & $0.033^{**}$ & $-0.034$\\

   
   \hline
\end{tabular}}
\caption{Beta coefficients for EEC inference for all model, valence, EEC combinations. Statistically significant results $(p \leq 0.01$) are marked with three asterisks ***, $(p \leq 0.05$) are marked with three asterisks **, $(p \leq 0.10$) are marked with three asterisks *}
\end{table*}

